Sampling of graph signals with successive local aggregations

A new scheme to sample signals defined in the nodes of a graph is proposed. The underlying assumption is that such signals admit a sparse representation in a frequency domain related to the structure of the graph, which is captured by the so-called graph-shift operator. Most of the works that have looked at this problem have focused on using the value of the signal observed at a subset of nodes to recover the signal in the entire graph. Differently, the sampling scheme proposed here uses as input observations taken at a single node. The observations correspond to sequential applications of the graph-shift operator, which are linear combinations of the information gathered by the neighbors of the node. When the graph corresponds to a directed cycle (which is the support of time-varying signals), our method is equivalent to the classical sampling in the time domain. When the graph is more general, we show that the Vandermonde structure of the sampling matrix, which is critical to guarantee recovery when sampling time-varying signals, is preserved. Sampling and interpolation are analyzed first in the absence of noise and then noise is considered. We then study the recovery of the sampled signal when the specific set of frequencies that is active is not known. Moreover, we present a more general sampling scheme, under which, either our aggregation approach or the alternative approach of sampling a graph signal by observing the value of the signal at a subset of nodes can be both viewed as particular cases. The last part of the paper presents numerical experiments that illustrate the results developed through both synthetic graph signals and a real-world graph of the economy of the United States.

==> figures/cyclic_graph.tex <==
\def \thisplotscale {1}
\def \unit {\thisplotscale cm}
\tikzstyle {blue vertex here} = [blue vertex, 
                                 minimum width = 0.5*\unit, 
                                 minimum height = 0.5*\unit, 
                                 anchor=center,
                                 font=\scriptsize]
{\small \begin{tikzpicture}[thick, x = 1.2*\unit, y = 0.96*\unit]

    
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%	
	% D R A W   N E T W O R K   %%%%%%%%%%%%
	%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\large
	  \node at (-1.5, 1.5)  {$\mathcal{G}_{dc}$};
	\small 
	
	% Draw radial nodes
	\node at (0,0) (center) {};
	\path (center) ++ (90:1.3) node (1) [blue vertex here] {1};
	\path (center) ++ (30:1.3) node (2) [blue vertex here] {2};
	\path (center) ++ (330:1.3) node (3) [blue vertex here] {3};
	\path (center) ++ (210:1.3) node (N-1) [blue vertex here] {N-1};
	\path (center) ++ (150:1.3) node (N) [blue vertex here] {N};
	
	% Draw invisible node for arrow out of node 3
	\path (center) ++ (290:1.5) node (3in) {};
	
	% Draw invisible node for arrow into node N-1
	\path (center) ++ (250:1.5) node (N-1in) {};

	% Draw dots
	\path (center) ++ (270:1.5) node (dots) {{\huge $\cdots$}};

	
	% Draw edges
	\path[thick, -stealth] (1) edge [bend left=20, above] node {{}} (2);		                            
	\path[thick, -stealth] (2) edge [bend left=20, above] node {{}} (3);		                            
	\path[thick, -stealth] (N-1) edge [bend left=20, above] node {{}} (N);		                            
	\path[thick, -stealth] (N) edge [bend left=20, above] node {{}} (1);		                            
	
	\path[thick, -stealth] (3) edge [bend left=20, above] node {{}} (3in);		                            
	\path[thick, -stealth] (N-1in) edge [bend left=20, above] node {{}} (N-1);		                            

	
      
\end{tikzpicture}}

==> sampling.tex <==
%!TEX root = SamplingSigGraphs_Draft.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\section{Sampling of graph signals}\label{S:Modeling}

Let $\ccalG=(\ccalN,\ccalE)$ denote a directed and unweighted graph. The set of nodes $\ccalN$ has cardinality $N$, and the set of links $\ccalE$ is such that  $(i,j)\in\ccalE$ if and only if node $i$ is connected to node $j$. The set $\ccalN_i:\{j\;\;|(j,i)\in\ccalE\}$ contains all nodes with an incoming connection to $i$ and is termed the incoming neighborhood of $i$. For any given graph we define the unweighted adjacency matrix $\bbA$ as a sparse matrix with nonzero elements $A_{ij}=1$ if and only if $(i,j)\in\ccalE$. The focus of this paper is not on analyzing $\ccalG$, but a graph signal defined on the set of nodes $\ccalN$. Such a signal can be represented as a vector $\bbx=[x_1,\ldots,x_N]^T \in  \mathbb{R}^N$ where the $i$-th component represents the value of the signal at node $i$, or, equivalently, as a function $f : \ccalN \to \mathbb{R}$, defined on the vertices of the graph.

%, the degree matrix as a diagonal matrix $\bbD$ with elements $((\bbD))_{ii}=\#(\ccalN_i)$ that contain the cardinality of incoming neighborhoods, and the Laplacian matrix as $\bbL:=\bbD-\bbA$.} \blue{Check that these are the definitions that we use.}

The graph $\ccalG$ is endowed with a \emph{graph-shift operator} $\bbS$ defined as an $N\times N$ matrix whose entry $(i,j)$, denoted as $s_{ij}$, is nonzero if and only if $i=j$ or $(i,j)\in\ccalE$. The sparsity pattern of the matrix $\bbS$ captures the local structure of $\ccalG$ but we make no specific assumptions on the values of the nonzero entries of $\bbS$. Common choices for $\bbS$ are the adjacency matrix of the graph \cite{SandryMouraSPG_TSP13,SandryMouraSPG_TSP14Freq}, its Laplacian \cite{EmergingFieldGSP}, and their generalizations \cite{GraphBook}. The intuitive interpretation of $\bbS$ is that it represents a linear transformation that can be computed locally at the nodes of the graph. If $\bby=[y_1,\ldots,y_N]^T$ is defined as $\bby=\bbS\bbx$, then node $i$ can compute $y_i$ provided that it has access to the values of $x_j$ at incoming neighbors $j\in \ccalN_i$. We assume henceforth that $\bbS$ is diagonalizable, so that there exist a matrix $\bbV\in\reals^{N\times N}$ and a diagonal matrix $\bbLambda\in\reals^{N\times N}$ that can be used to decompose $\bbS$ as
%
\begin{equation}\label{eqn_eigendecomposition}
   \bbS=\bbV\bbLambda\bbV^{-1}.
\end{equation}
%
In particular, \eqref{eqn_eigendecomposition} is true for normal matrices satisfying $\bbS\bbS^H=\bbS^H\bbS$. In that case we have that $\bbV$ is orthonormal, which implies $\bbV^{-1}=\bbV^{H}$, and leads to the decomposition $\bbS=\bbV^H\bbLambda\bbV$.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure}
\centering
\input{figures/graph_palette}
\input{figures/regular_sampling.tex}
\caption{Sampling in the time domain as selection sampling on a directed cycle graph. Discrete time domain can be represented by a cyclic graph connecting node $i$ to $i+1$ and node $N$ to node 1. Using the uniform selection matrix $\bbC=[\bbe_1,\bbe_{N/K+1},\ldots,\bbe_{N-N/K+1}]^T$ with $K/N=1/2$ results in the selection of all even signals $x_1,x_3,\ldots,x_{N-1}$. Observe that this sampling rule is independent of the structure of the underlying graph.}
\label{fig_selection_sampling}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   M   A   I   N       M   A   T   T   E   R   %%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
A natural definition of sampling for a graph signal is to introduce a fat selection
matrix $\bbC\in\reals^{K\times N}$ and define the sampled signal as \cite{SamplingKovacevicMoura_1415}
%
\begin{equation}\label{eqn_selection_sampling}
   \tbx_s = \bbC\bbx.
\end{equation}
%
If the matrix $\bbC$ is chosen as binary, i.e., with elements $c_{ij}\in\{0,1\}$; having a single nonzero element per row; and at most one nonzero element per column; the signal $\tbx$ is a selection of $K$ out of the $N$ elements of $\bbx$. In such case the ratio $K/N$ is the sampling rate of the signal. Uniform sampling amounts to setting \green{$\bbC=[\bbe_1,\bbe_{N/K+1},\ldots,\bbe_{N-N/K+1}]^T$} and the selection of the first $K$ elements of $\bbx$ is accomplished by setting $\bbC=\bbE_K:=[\bbe_1,\ldots,\bbe_{K}]^T$. We remark that, in general, it is not clear how to choose good selection matrices $\bbC$. This is in contrast to conventional sampling of signals in the time domain where uniform sampling is advantageous.

An equally valid, if less intuitive, definition is to fix a node, say $i$, and consider the sampling of the signal seen by this node as the shift operator $\bbS$ is applied recursively. To describe this sampling methodology better, define the $l$th shifted signal $\bby^{(l)}:=\bbS^l\bbx$ and further define the matrix
%
\begin{equation}\label{eqn_all_shifts_matrix}
   \bbY\,:=\,[\bby^{(0)},\bby^{(1)},\ldots,\bby^{(N-1)}]
       \,:=\,[\bbx,\bbS\bbx,\ldots,\bbS^{N-1}\bbx],
\end{equation}
%
that groups the signal $\bbx$ and the result of the first $N-1$ applications of the shift operator. Associating the $i$th row of $\bbY$ with node $i$, we define the successively aggregated signal at $i$ as $\bby_i:=(\bbe_i^T\bbY)^T=\bbY^T\bbe_i$. Sampling is now reduced to the selection of $K$ out of the $N$ rows of $\bby_i$, which we accomplish with a selection matrix $\bbC$ [cf. \eqref{eqn_selection_sampling}]
%
\begin{equation}\label{eqn_aggregation_sampling}
   \bbx_s \ :=\ \bbC\bby_i\ =\ \bbC \left(\bbY^T\bbe_i\right).
\end{equation}
%
We say that the signal $\bbx_s$ samples $\bbx$ with successive local aggregations. This nomenclature follows from the fact that $\bby^{(l)}$ can be computed recursively as $\bby^{(l)}:=\bbS\bby^{(l-1)}$ and that the $i$th element of this vector can be computed using signals associated with itself and its incoming neighbors,
%
\begin{equation}\label{eqn_local_aggregation}
   y^{(l)}_i = \sum_{j\in\ccalN_i} S_{ij} y^{(l-1)}_j.
\end{equation}
%
We can then think of the signal $\bby_i$ as being computed locally at node $i$ using successive variable exchanges with neighboring nodes. In fact, it is easy to show that $y_i^{(l)}$ can be expressed as a linear combination of the values of $x_j$ at nodes $j$ whose distance (number of hops) from node $i$ is less than or equal to $l$. This implies that the sampled signal $\bbx_s$ in \eqref{eqn_aggregation_sampling} is a selection of values that node $i$ can determine locally. An underlying idea behind the sampling in \eqref{eqn_aggregation_sampling} is to incorporate the structure of the shift into the sampling procedure. Both $\mathbf{S}$ and  $\mathbf{y}^{(l)}$ play key roles in other graph-processing algorithms such as shift-invariant graph filters \cite{SandryMouraSPG_TSP13}, where the output of the filter is a linear combination of the shifted signals $\mathbf{y}^{(l)}$.



To understand the difference between selection sampling [cf. \eqref{eqn_selection_sampling}] and aggregation sampling [cf. \eqref{eqn_aggregation_sampling}], it is instructive to consider their application to a signal defined in the time domain. We do so in the following section.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   F   I   G   U   R   E   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\begin{figure*}
\centering
\input{figures/graph_palette}
\input{figures/cyclic_sampling.tex}
\caption{Sampling in the time domain as aggregation sampling in a directed cycle graph. In aggregation sampling we utilize successive applications of a shift operator determined by the given graph and sample the resulting signal observed at a given node. Using the cycle adjacency matrix $\bbA_c$ as shift operator results in the signal $\bbx$ rotating through the graph and the selection of elements of the aggregated signal reduces to conventional sampling. Aggregation sampling is, therefore, a generalization of conventional sampling to graph signals that utilizes the underlying graph structure in the construction of samples.}
\label{F:DirectedChainGraph_sampling}
\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%   S   E   C   T   I   O   N   %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\subsection{Example: Sampling in the time domain}

Classical time domain signals can be represented as graph signals defined on top of a directed cycle graph; see Figure \ref{fig_selection_sampling}. To do so define the cycle graph $\ccalG_{c}$ as one in which the edge set $\ccalE_{c}:=\{(i,\mymod(i)+1)\}_{i=1}^N$, connects node $i$ to node $i+1$ for all nodes except $N$, which is connected to node 1. The elements of the adjacency matrix of this graph, denoted as $\bbA_{c}$, are zero except for the ones in the first cyclic superdiagonal, which are one.

For a signal $\bbx$ defined on top the directed cycle $\ccalG_{c}$, we consider selection sampling and aggregation sampling when using the shift operator $\bbS=\bbA_{c}$ and the uniform selection matrix $\bbC=[\bbe_1,\bbe_{N/K+1},\ldots,\bbe_{N-N/K+1}]^T$. Illustrations of the respective sampling procedures are available in figures \ref{fig_selection_sampling} and \ref{F:DirectedChainGraph_sampling} for a signal with $N=6$ elements and sampling rate $K/N=1/2$.

In selection sampling we just multiply the graph signal $\bbx$ with the selection matrix $\bbC$ to obtain the sampled signal $\tbx_s = \bbC\bbx$ as indicated by \eqref{eqn_selection_sampling}. In aggregation sampling we consider subsequent applications of the shift matrix $\bbS=\bbA_c$. Each of these shifts amounts to rotating the signal clockwise so that the element at node $i$ moves to node $i+1$ for all $i<N$ and the element at node $N$ moves to node $1$. If we consider, e.g., node $i=1$, the first shift moves signal $x_{N}$ to this node so that $y_{1}^{(1)}=x_N$, the second shift moves signal $x_{N-1}$ so that $y_{1}^{(2)}=x_{N-1}$ and so on. It follows that the aggregated signal $\bby_1$ in \eqref{eqn_all_shifts_matrix} is given by $\bby_1=[x_1, x_{N}, x_{N-1},\ldots,x_2]$. This is just a shift of the original signal $\bbx$, which, upon multiplication by the selection matrix $\bbC$ as per \eqref{eqn_aggregation_sampling} results in a vector $\bbx_s:=\bbC\bby_1$ that contains the same elements that $\tbx_s$ contains.

For the cycle graph and shift operator $\bbS=\bbA_c$ selection and aggregation sampling produce not only equivalent sampled signals but also reduce to conventional sampling. This is not a coincidence because both methods are designed as generalizations of conventional sampling. In general, selection sampling and aggregation sampling produce different outcomes. In selection sampling we move through nodes to collect samples at points uniquely identified by $\bbC$, whereas in aggregation sampling we move the signal through the graph while collecting samples at a fixed node. Observe that because aggregation sampling depends on the shift operator, it incorporates the structure of the graph into the sampling procedure. This is not true of selection sampling except for the selection of matrices $\bbC$ adapted to particular graphs.

%\red{More precisely, we can say that our sampling process includes a preprocessing based on the sequential application of $\bbS$ --related to, e.g., the notions of smoothing kernels \cite{VetterliFRI_TSP02}. The shift operator $\bbS$ and the shifted signals $\bby^{(l)}$ also play key roles in other graph-processing algorithms such as shift-invariant graph filters \cite{SandryMouraSPG_TSP13}, where the output of the filter is a linear combination of the columns of $\bbY$.} \blue{Can we remove this?}


